Negative binomial count splitting for single-cell RNA sequencing data

The analysis of single-cell RNA sequencing (scRNA-seq) data often involves fitting a latent variable model to learn a low-dimensional representation for the cells. Validating such a model poses a major challenge. If we could sequence the same set of cells twice, we could use one dataset to fit a latent variable model and the other to validate it. In reality, we cannot sequence the same set of cells twice. Poisson count splitting was recently proposed as a way to work backwards from a single observed Poisson data matrix to obtain independent Poisson training and test matrices that could have arisen from two independent sequencing experiments conducted on the same set of cells. However, the Poisson count splitting approach requires that the original data are exactly Poisson distributed: in the presence of any overdispersion, the resulting training and test datasets are not independent. In this paper, we introduce negative binomial count splitting, which extends Poisson count splitting to the more flexible negative binomial setting. Given an $n \times p$ dataset from a negative binomial distribution, we use Dirichlet-multinomial sampling to create two or more independent $n \times p$ negative binomial datasets. We show that this procedure outperforms Poisson count splitting in simulation, and apply it to validate clusters of kidney cells from a human fetal cell atlas.

==> sections/extra_intuition.tex <==
%\section{Additional intuition for beta-binomial thinning when $b$ and $\epsilon b$ are both integers.}
%\label{appendix_integer_intuition}

%Recall that if $\by \sim \NB\left( \mu, b \right)$ and $b$ is an integer, then we can interpret $\by$ as the number of successes that occur in a sequence of i.i.d. $\mathrm{Bernoulli}\left(\frac{\mu}{b+\mu}\right)$ trials before $b$ failures occur. This means that $\by$ is the sum of $b$ independent $\text{Geom}\left(\frac{\mu}{b+\mu}\right)$ random variables. 


%If $\epsilon b$ and $(1-\epsilon) b$ are both integers, then we know that the 


%we can view the thinning procedure from Theorem~\ref{theorem_nbthin} as decomposing $\by$ into the $\bytr$ successes that occurred before the first $\epsilon b$ failures, and then the remaining $\byte$ successes. This interpretation lends itself to a derivation of the beta-binomial thinning procedure.





%Since $\bx=X$ is fixed, we know for sure 

%We imagine an urn with $b+X-1$ total elements in it, of which $X$ are labeled ``successes" and $b-1$ are labeled as failures. \textcolor{red}{do I need to explain why we only want $b-1$ and not $b$ in the urn? It's clear to me if I draw a more }


%Since $\bx=X$ is now fixed, to simulate which successes occurred before the first $b_1$ failures we should draw WITHOUT REPLACEMENT from this urn until we draw 

%When $b, \epsilon b$, and $(1-\epsilon)b$ are all integers, the distribution $\bb(X,\epsilon b, (1-\epsilon)b)$ is the \emph{negative hypergeometric} distribution with parameters $b+X-1$, $X$, and $\epsilon b$. \textcolor{red}{do I need a source that is not wikipedia + my pen and pencil???} The interpretation of drawing $\bxtr \mid bx = X \sim \mathrm{NegHyp(b+X-1, X, \epsilon b})$ is clear. 

